A Centralized Multi-stage Non-parametric Learning Algorithm for Opportunistic Spectrum Access

Owing to the ever-increasing demand in wireless spectrum, Cognitive Radio (CR) was introduced as a technique to attain high spectral efficiency. As the number of secondary users (SUs) connecting to the cognitive radio network is on the rise, there is an imminent need for centralized algorithms that provide high throughput and energy efficiency of the SUs while ensuring minimum interference to the licensed users. In this work, we propose a multi-stage algorithm that - 1) effectively assigns the available channel to the SUs, 2) employs a non-parametric learning framework to estimate the primary traffic distribution to minimize sensing, and 3) proposes an adaptive framework to ensure that the collision to the primary user is below the specified threshold. We provide comprehensive empirical validation of the method with other approaches.

==> figs/plots_template.tex <==
\addplot[black, solid, thick, 
                mark=-, mark size={3.0}, mark phase=1, mark repeat=3
                ] 
            table [x=Genie_Genie_x, y=Genie_Genie_y, col sep=comma]{\datatable};
        \addlegendentry{Genie};

        \addplot[black, solid, thick, 
                mark=o, mark size={3.0}, mark phase=1, mark repeat=3
                ] 
            table [x=Genetic_SenseAlways_x, y=Genetic_SenseAlways_y, col sep=comma]\datatable;
        \addlegendentry{Sense Always};

        \addplot[black, solid, thick, 
                mark=asterisk, mark size={3.0}, mark phase=1, mark repeat=3
                ] 
            table [x=Genetic_TUC_x, y=Genetic_TUC_y, col sep=comma]{\datatable};
        \addlegendentry{TUC};
        
        \addplot[black, solid, thick, 
                mark=|, mark size={3.0}, mark phase=1, mark repeat=3
                ] 
            table [x=Genie_Raj2018_x, y=Genie_Raj2018_y, col sep=comma]{\datatable};
        \addlegendentry{Genie aided \cite{raj2018spectrum}};
        
        % \addplot[black, solid, thick, 
        %         mark=diamond, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
        %         ] 
        %     table [x=Genetic_Raj2018_x, y=Genetic_Raj2018_y, col sep=comma]\datatable;
        % \addlegendentry{Hill Climbing aided \cite{raj2018spectrum}};


        % \addplot[black, solid, thick, 
        %         mark=star, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
        %         ] 
        %     table [x=Genetic_Proposed_FDSA_Sq_x, y=Genetic_Proposed_FDSA_Sq_y, col sep=comma]\datatable;
        % \addlegendentry{Proposed FDA ($y^2$)};
        
        \addplot[black, solid, thick, 
                mark=square, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
                ] 
            table [x=Genetic_Proposed_Fixed_eps_0_1_x, y=Genetic_Proposed_Fixed_eps_0_1_y, col sep=comma]\datatable;
        \addlegendentry{Proposed with $\epsilon = 0.10$)};
        
        \addplot[black, solid, thick, 
                mark=oplus, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
                ] 
            table [x=Genetic_Proposed_FDSA_SqExp_x, y=Genetic_Proposed_FDSA_SqExp_y, col sep=comma]\datatable;
        \addlegendentry{Proposed FDSA ($y^2\&\exp(y)$)};
        
        % \addplot[black, solid, thick, 
        %         mark=otimes, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
        %         ] 
        %     table [x=Genetic_Proposed_FDSA_Exp_x, y=Genetic_Proposed_FDSA_Exp_y, col sep=comma]\datatable;
        % \addlegendentry{Proposed FDA ($\exp(y)$)};
        
        % \addplot[black, solid, thick, 
        %         mark=triangle, mark size={3.0}, mark color=black, mark phase=1, mark repeat=3
        %         ] 
        %     table [x=Genetic_Proposed_Decreasing_eps_x, y=Genetic_Proposed_Decreasing_eps_y, col sep=comma]\datatable;
        % \addlegendentry{Proposed (decreasing $\epsilon$)};
        
        
